OpenResearcher: A Fully Open Pipeline for Long-Horizon Deep Research Trajectory Synthesis

Training deep research agents requires long-horizon trajectories that interleave search, evidence aggregation, and multi-step reasoning. However, existing data collection pipelines typically rely on proprietary web APIs, making large-scale trajectory synthesis costly, unstable, and difficult to reproduce. We present OpenResearcher, a reproducible pipeline that decouples one-time corpus bootstrapping from multi-turn trajectory synthesis and executes the search-and-browse loop entirely offline using three explicit browser primitives: search, open, and find, over a 15M-document corpus. Using GPT-OSS-120B as the teacher model, we synthesize over 97K trajectories, including a substantial long-horizon tail with 100+ tool calls. Supervised fine-tuning a 30B-A3B backbone on these trajectories achieves 54.8\% accuracy on BrowseComp-Plus, a +34.0 point improvement over the base model, while remaining competitive on BrowseComp, GAIA, and xbench-DeepSearch. Because the environment is offline and fully instrumented, it also enables controlled analysis, where our study reveals practical insights into deep research pipeline design, including data filtering strategies, agent configuration choices, and how retrieval success relates to final answer accuracy. We release the pipeline, synthesized trajectories, model checkpoints, and the offline search environment at https://github.com/TIGER-AI-Lab/OpenResearcher.

==> cases/case10.tex <==
\subsection{Case 9: Failure from xbench (Found Data, Wrong Extraction)}

\model retrieves all of the evidence needed from Chinese Wikipedia (12 searches, 37 opens, 6 finds) but still reports an incorrect count, because its enumeration over that evidence is incomplete. As early as Turn 3, a single \texttt{find} call already surfaces the full list of Heilongjiang's 13 prefecture-level divisions---including 鸡西、鹤岗、双鸭山、伊春、佳木斯、牡丹江、黑河 and 大兴安岭地区, eight of which border Russia---yet the model verifies only four of them one by one and then treats its enumeration as complete. It repeats the same partial sweep for Jilin, counting only 延边 while dropping 白山 and 通化 even though both appeared in observations it had already read, and closes with $4+1+1=6$ against a gold answer of 12. The thinking traces show the model parsing large administrative tables and arriving at a plausible but wrong total, highlighting that precise extraction from dense pages---not retrieval---is the binding constraint here.

\begin{custombox}[title=Example from xbench]

\textbf{Question:} 黑龙江、吉林、辽宁，共有多少个地市级行政单位与外国接壤？

\vspace{1em}

\textbf{Answer:} 12
\end{custombox}

\begin{casebox}{failbg}{failframe}{Failure Case Study (12 search + 37 open + 6 find)}

    \textbf{Turn 1:}

    \textbf{Reasoning Content:} We need to answer the question: ``黑龙江、吉林、辽宁，共有多少个地市级行政单位与外国接壤？'' [...] The phrase ``地市级行政单位'' refers to prefecture-level city administrative units, i.e., prefecture-level cities (including municipalities, prefecture-level cities, and also possibly autonomous prefectures?)...

    \vspace{0.3em}

    \begin{itemize}[nosep, leftmargin=*, label={}]
        \item \textbf{Tool:} \smalltt{search}
        \item \textbf{Tool Call:}

        \smalltt{\{"query": "黑龙江 地市 与 外国 接壤", "topn": 10\}}
        \item \textbf{Result:}
        \begin{casecode}{failbg}
[0] 黑龙江 地市 与 外国 接壤 (web-search://ts=1769809477)
**viewing lines [0 - 26] of 26**

L0:
L1: URL: web-search://ts=1769809477
L2: \# Search Results
L3:
L4:   * [0†黑龍江省 - 維基百科，自由的百科全書†zh.wikipedia.org]
L5: 省界東、北與俄羅斯接壤，南接吉林省，西鄰內蒙古自治區 ...
        \end{casecode}
    \end{itemize}
    \vspace{1em}


    \textbf{Turn 3} \textit{(the complete evidence is already on screen here)}\textbf{:}

    \textbf{Reasoning Content:} Scrolling for border discussion.

    \vspace{0.3em}

    \begin{itemize}[nosep, leftmargin=*, label={}]
        \item \textbf{Tool:} \smalltt{find}
        \item \textbf{Tool Call:}

        \smalltt{\{"cursor": 1, "pattern": "地级"\}}
        \item \textbf{Result:}
        \begin{casecode}{failbg}
[2] Find results for text: `地级` in `黑龙江省 - 维基百科，自由的百科全书`
(https://zh.wikipedia.org/wiki/黑龙江省/find?pattern=地级)
**viewing lines [0 - 25] of 28**

L6: \# [1†match at L89]
L7: 行政区划 黑龙江省现辖12个地级市、1个地区，下设54个市辖区、21个县级市、45个县、
L8: 1个自治县 [...]
L9: 地级市：哈尔滨市（行政级別为副省级）、齐齐哈尔市、鸡西市、鹤岗市、双鸭山市、
L10: 大庆市、伊春市、佳木斯市、七台河市、牡丹江市、黑河市、绥化市 * 地区：大兴安岭地区
        \end{casecode}
    \end{itemize}
    \vspace{1em}

    \vspace{0.5em}
    $\cdots$

    \textbf{Turns 4--54}: 51 additional tool calls omitted --- the model verifies the border status of only four Heilongjiang cities (黑河、伊春、佳木斯、牡丹江) one at a time, then moves on to Jilin and Liaoning $\cdots$
    \vspace{0.5em}

    \textbf{Turn 55:}

    \textbf{Reasoning Content:} Now Dandong page lines 12-14 show border with North Korea. Let's capture.

    \vspace{0.3em}

    \begin{itemize}[nosep, leftmargin=*, label={}]
        \item \textbf{Tool:} \smalltt{open}
        \item \textbf{Tool Call:}

        \smalltt{\{"cursor": 32, "loc": 12\}}
        \item \textbf{Result:}
        \begin{casecode}{failbg}
[40] 丹东市 - 维基百科，自由的百科全书 (https://zh.wikipedia.org/wiki/丹东市)
**viewing lines [12 - 27] of 192**

L12: 丹东市，旧称安东，是中华人民共和国辽宁省下辖的地级市，辽宁省重要的边境口岸和
L13: 辽东地区中心城市 [...] 东与朝鲜民主主义人民共和国平安北道新義州市隔江相望[1]。
L15: [...] 丹东是中国最大的边境城市 ...
        \end{casecode}
    \end{itemize}
    \vspace{1em}


    \textbf{Final Answer:} In Heilongjiang province the prefecture-level cities that touch a foreign country are \textbf{Heihe}, \textbf{Yichun}, \textbf{Jiamusi} and \textbf{Mudanjiang} --- that gives \textbf{4} units. In Jilin province the only prefecture-level unit that borders a foreign country is the \textbf{Yanbian Korean Autonomous Prefecture}, which shares borders with both Russia and North Korea --- \textbf{1} unit. In Liaoning province the sole prefecture-level city that borders a foreign country is \textbf{Dandong}, which faces North Korea across the Yalu River --- \textbf{1} unit. Adding them up: $4+1+1=\mathbf{6}$ prefecture-level administrative units that share a border with a foreign country. {Exact Answer:} 6.

    \textbf{Confidence: 95\%}

\end{casebox}

